GrandCode: Achieving Grandmaster Level in Competitive Programming via Agentic Reinforcement Learning

Competitive programming remains one of the last few human strongholds in coding against AI. The best AI system to date still underperforms the best humans competitive programming: the most recent best result, Google's Gemini~3 Deep Think, attained 8th place even not being evaluated under live competition conditions. In this work, we introduce GrandCode, a multi-agent RL system designed for competitive programming. The capability of GrandCode is attributed to two key factors: (1) It orchestrates a variety of agentic modules (hypothesis proposal, solver, test generator, summarization, etc) and jointly improves them through post-training and online test-time RL; (2) We introduce Agentic GRPO specifically designed for multi-stage agent rollouts with delayed rewards and the severe off-policy drift that is prevalent in agentic RL. GrandCode is the first AI system that consistently beats all human participants in live contests of competitive programming: in the most recent three Codeforces live competitions, i.e., Round~1087 (Mar 21, 2026), Round~1088 (Mar 28, 2026), and Round~1089 (Mar 29, 2026), GrandCode placed first in all of them, beating all human participants, including legendary grandmasters. GrandCode shows that AI systems have reached a point where they surpass the strongest human programmers on the most competitive coding tasks.

==> header_style.tex <==
% 一次性加载 geometry，给出页边距和 \headheight
% 增加 headsep 来让第一页页眉和正文之间有更大间距
\usepackage[margin=3cm, headheight=50pt, headsep=0pt]{geometry}

\usepackage{graphicx}   % 插图
\usepackage{fancyhdr}   % 自定义页眉页脚

% ------- 页眉定义 -------
\pagestyle{fancy}       % 默认页眉样式
\fancyhf{}              % 清空

% 删除默认页面的横线
\renewcommand{\headrulewidth}{0pt}

\begin{comment}
% 左侧：logo + 项目名，可按需删掉 \textsc{}
\fancyhead[L]{%
  \raisebox{-0.25\height}{\includegraphics[height=20pt]{./header.png}}%
}

% 右侧放页码示例（可不要）
\fancyhead[R]{}

% (2) 横向"拉长"：把页眉区域往左右各伸出 2.5 cm
\fancyheadoffset[L]{0.2cm}
\fancyheadoffset[R]{0.2cm}
\end{comment}

% 让首页 (plain) 同样使用这种页眉
\fancypagestyle{plain}{%
  \fancyhf{}
  \fancyhead[L]{%
    % 方法1：通过添加 \vspace 来让页眉内容下移
    \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{\includegraphics[height=25pt]{./header.png}}%
      \vfill
    }%
  }
  \fancyhead[R]{
  \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{}
      \vfill
    }%
  }
  \renewcommand{\headrulewidth}{0.7pt}  % 保留第一页的横线
  \fancyheadoffset[L]{0cm}
  \fancyheadoffset[R]{0cm}
}

% 如果只想让第一页的页眉和正文间距更大，可以在文档开始处使用：
% \thispagestyle{plain}
% \vspace{20pt}  % 在第一页正文开始前添加额外空间
